A hyper-runaway white dwarf in Gaia DR2 as a Type Iax supernova primary remnant candidate

Observations of stellar remnants linked to Type Ia and Type Iax supernovae are necessary to fully understand their progenitors. Multiple progenitor scenarios predict a population of kicked donor remnants and partially-burnt primary remnants, both moving with relatively high velocity. But only a handful of examples consistent with these two predicted populations have been observed. Here we report the likely first known example of an unbound white dwarf that is consistent with being the fully-cooled primary remnant to a Type Iax supernova. The candidate, LP 93-21, is travelling with a galactocentric velocity of v$_{gal}$ $\simeq$ 605 km s$^{-1}$, and is gravitationally unbound to the Milky Way. We rule out an extragalactic origin. The Type Iax supernova ejection scenario is consistent with its peculiar unbound trajectory, given anomalous elemental abundances are detected in its photosphere via spectroscopic follow-up. This discovery reflects recent models that suggest stellar ejections likely occur often. Unfortunately the intrinsic faintness of white dwarfs, and the uncertainty associated with their direct progenitor systems, makes it difficult to detect and confirm such donors.

==> motivation.tex <==
\section{Motivation for expected observables} \label{motivation}

In this section we present a short summary of the most likely observational signatures associated with a DR from a handful of the most likely SNe Ia progenitor scenarios. We also present an estimate to the number of DRs we would expect in our observable volume within the Milky Way.

\subsection{Donor remnants to SNe Ia}

Tidbit here about how both SD and DD are thought to contribute to the rate of all SNe Ia and even SNe Iax??? **

\subsubsection{Double-denegerate remnants}

%Most, if not all, SNe Ia leave an intact companion DR.

Although the exact progenitors to SNe Ia remain uncertain, a sub-Chandrasekhar (sub-Ch) mass C/O WD accreting helium-rich mass from a WD companion in the DD scenario is one possible pathway (see \cite{Maoz2014} for a review). There is now evidence to suggest all DD WD systems eventually undergo dynamically \textit{unstable} mass transfer, even those that eventually coalesce to form a single merger remnant \citep{Pakmor2013, Shen2015, Danetal2015}. Unstable mass transfer may trigger a helium shell detonation in the primary WD and a subsequent detonation in its core during the initial phases of mass transfer, leading to a SN Ia well before complete tidal disruption of the companion WD \citep{ShenMoore2014, ShenSchwab2017}. This is the so-called ``double-detonation’’ channel thought to occur in the large majority of DD SNe Ia (also known as the ``D$^6$'' scenario or ``helium-ignited violent merger model’’, see \cite{Pakmor2013, Shen2018b, Shen2018a}). Dynamically \textit{stable} mass transfer to the primary WD is also possible \citep{Bildstenetal2007, ShenBildsten2009}, and can lead to a helium shell detonation with subsequent core detonation in a variant of the double-detonation scenario.

The double-detonation channel implies the companion WD survives the explosion of the primary in either stability regime, leaving a surviving DR traveling at high velocity \citep{Shen2015, ShenSchwab2017, Tanikawa2018}. This is supported by observational constraints. If the companion WD were to fully tidally disrupt, it should form a torus surrounding the primary WD \citep{Danetal2014}. This torus should cause significant asymmetry to the SN Ia ejecta -- which is directly at odds with the high levels of symmetry found in SNe Ia remnants \citep{Bulla2016}. The material in the torus surrounding the primary WD should also pollute the SN Ia ejecta. This material should be observable by emission lines but is almost never detected \citep{Shen2018b}.

The double-detonation channel also implies different effects (over different timescales) for the DR in either SNe Ia mass transfer stability regime. For the unstable regime, shock heating from the SN Ia and its ejecta, tidal field heating, and the capture, accretion, and delayed radioactive decay of $^{56}$Ni $\longrightarrow$ $^{56}$Co $\longrightarrow$ $^{56}$Fe likely affect the outer layers of the companion WD \citep{ShenSchwab2017, Tanikawa2018}. These effects manifest by increasing the luminosity of the WD DR (i.e. $>$\,0.1 L$_{\odot}$) and causing the colour to become bluer than expected anywhere from a few years to a few centuries \citep{Iben1998, ShenSchwab2017, Shen2018b}. By extension, these effects are therefore important mostly in discriminating younger DRs from ``local’’, historical SNe Ia rather than older DRs with ambiguous origins. For the stable regime, the donor is only mildly distorted by these effects and should return to the WD cooling sequence much sooner.

% not sure why but this paragraph won't let the entire document compile
\citet{Tanikawa2018} simulate the interaction between, and the evolution of, a primary 1.0 M$_{\odot}$ C/O WD with a large He shell and a secondary 0.6 M$_{\odot}$ C/O WD. The He shell on the primary WD was artificially thick so that the He and subsequent C/O detonation would succeed easily. \citet{Tanikawa2018} followed the evolution of the binary system from the initiation of the He detonation to the effects of the SN Ia ejecta on the expected DR observables. The DR's mass remains roughly equal, but it does capture a small amount of material originating from the centre of the detonation in the primary WD (the slowest ejected material, most easily caught by the companion, should originate from the densest region). This material consists mostly of $^{56}$Ni and He because when a C/O detonation propagates through a high-density region it mostly synthesises $^{56}$Ni, and a small amount of He is left as a residual due to photo-dissociation. \citet{Tanikawa2018} found the DR WD contaminated with approximately 0.03 M$_{\odot}$ of $^{56}$Ni and 3\,$\times$\,10$^{-4}$ M$_{\odot}$ He, which is similar to the results of \citet{ShenSchwab2017}, the only other cited simulation following the D$^6$ SN Ia scenario and the subsequent ejecta impact on DR observables.

The $^{56}$Ni will undergo delayed radioactive decay $^{56}$Ni $\longrightarrow$ $^{56}$Co $\longrightarrow$ $^{56}$Fe within the DR \citep{ShenSchwab2017}. The decaying $^{56}$Ni can be identified as anomalous, but it is still unclear if the material stays on the surface of the DR due to radiative levitation \citep{Chayer1995a, Chayer1995b} or falls to the centre due to sedimentation \citep{Paquette1986, Dupuis1992}. It is necessary to perform further simulations to follow the time evolution of the DR to know whether or not decay products remain on the surface of the WD, and if so,en how long they might impact late-time observations.

%Include paragraph(s) here laying out the extreme velocity distribution of these objects from this scenario and why they're so fast/extreme. Include Shen et al. (2018) calculation for expected number of D6 WDs here or mention it before our own calculation?

\citet{Shen2018b} model the runaway velocities of DRs produced by the D$^6$ scenario. \citet{Shen2018b} use the results of \citet{ShenSchwab2017} and \citet{Shen2018a} to assume the runaway velocity of the donating WD (both He and C/O WDs in their simulations) at the point of SN Ia is roughly equal to the orbital velocity of the companion star during Roche-lobe overflow. It is found the runaway velocities of surviving D$^6$ DRs are remarkable, in every case more than 1,000 km s$^{-1}$. For the case of a 0.6\,$M_{\odot}$ companion WD to a 1.0\,$M_{\odot}$ primary WD, the DR runaway velocity is found to be 1800 km s$^{-1}$. For the case of a near-equal mass binary of a 1.0\,$M_{\odot}$ companion and a 1.0\,$M_{\odot}$ primary, the DR runaway velocity is found to be an astounding 2,200 km s$^{-1}$.

The visual changes from the SN and its ejecta should last on the order of tens to hundred of years for local DD DRs originating from the Milky Way. It is still unknown if the captured SN ejecta is easily observable on the surface of the DR at late-time observations. Therefore the most distinguishing property of a DR originating from either a Milky Way or extragalactic SN Ia in the DD scenario is its exceptional space velocity.

% don't put observed D6 remnants here, put it in the discussion

\subsubsection{Single-denegerate remnants}

The SD scenario is another possible SNe Ia progenitor channel, in which a sub-Ch mass C/O WD accretes either hydrogen- or helium-rich mass through Roche-lobe overflow, or through a strong wind, from the companion to reach Ch-mass and detonate as a SN Ia (see \citet{Maoz2014} for a review). The donating companion may be a main-sequence (MS) hydrogen burning star (H-star), naked helium star (He-star, often called a ``(hot) subdwarf'' due to its hydrogen envelope being stripped off by binary interaction), or red giant (RG). Different configurations for either secondary can lead to a detonation of the primary WD, but each case depends on the previous common envelope and mass transfer phases. The survival of an intact companion star in the SD scenario is also expected from theoretical simulations and observational constraints \citep{}. In the same way as before, the intact companion from the SD scenario should display evidence of the explosion in its atmosphere \citep{} and be a kinematic outlier \citep{}.

% marietta et all 2008, pakmor et all 2008

Regardless of the sub-channel, the main SD channel predicts the primary sub-Ch mass WD will accrete matter from the companion star and increase in mass to approach the Chandreskhar-mass limit ($\approx$1.44\,$M_{\odot}$). Once it reaches this mass limit, the primary reaches sufficient density at the core to initiate a thermonuclear runaway explosion. This neatly explains the uniformity of supernovae remnant (SNR) light curves observed \citep{}. But for MS H-star companions, only a fairly narrow range in accretion rates above 10$^{-7}\,M_{\odot}$ yr$^{-1}$ are allowed for stable hydrogen mass transfer and burning on the surface of the primary WD, which allow the primary to avoid a regular nova explosion \citep{}. This narrow window heavily restricts possible H-star companion configurations leading to SN Ia.

Observed DRs possibly originating from the H-star companion SD channel are still in question, whereas a few promising DD channel DRs have been presented, providing further evidence for the difficulty H-stars have in producing SNe Ia \citep{}. SNe Ia SNRs are also characterised by a lack of hydrogen in their spectra, which is naturally explained by the DD channel. But in the hydrogen-accretion model of the SD scenario, simulations suggest the impact of the SN may strip off $\sim 0.03-0.15$ $M_{\odot}$ of H-rich material from H-star companions and almost entirely removes the envelop of RG companions, polluting the SN ejecta with hydrogen \citep{}. This is directly at odds with observations as well. High-resolution spectroscopy of two relatively hydrogen-rich extraglactic SNe Ia estimated an upper limit of only 0.01\,$M_{\odot}$ possible for the amount of stripped hydrogen polluting the ejecta \citep{}.

In addition to the difficulty of H-star companions leading to SN Ia, and observational constraints indicating SNe Ia are unlikely byproducts of H-rich mass transfer, simulations also suggest that the SN Ia effects on the companion H-star would also make it difficult to detect large visual differences at late-time observations (as evolved DRs).
%1) ejecta and luminosity/radius/evolution
**Tidbit here about how the ejecta will affect the luminosity and visuals of the MS H-star on short-ish timescales
%2) thermal bloat and luminosity
In the long pre-explosion mass transfer phase associated with H-rich accretion, the companion is pushed out of thermal equilibrium. The increased radius and luminosity of the companion arising from mass transfer in a binary system is known as ``thermal bloating'' \citep{Knigge2011}, but it is unlikely this effect lasts longer than the timescales associated with captured ejecta decay.
%3) SHORT what would we expect to see (thus also expect to see in WD remnant? Not necessarily?)
Still unknown  about the radiative levitation/settling - need more simulations!

**Although spin may be used as another diagnostic, apart from abundances. Jury's still out.

**The kinematics associated with H-star DRs also likely makes it difficult to detect them apart from background stars. --> Not fast enough to make them out on tangential velocity, which should be ``easy'' in big tangential velocity surveys. Not really fast enough in radial velocity alone either, and RV measurements are much less prevalent.

Following the difficulty of hydrogen-mass accretion in the SD scenario and the likely small, relatively difficult to distinguish (by abundances or kinematics) population of DRs associated with the hydrogen-mass accretion model, more attention in the past decade has been placed on the \textit{helium}-accretion model of the SD scenario \citep{}. It has been found that the He-star companion model to the SD channel can possibly describes the discrepancy in theory and observations for both SD and DD SNe Ia \citep{}. It has also been found to be a likely dominant pathway to the formation of (massive) DD systems \citep{}.

**He-mass transfer is easier for WDs \citep{}, hydrogen envelope can easily be stripped off via binary interaction \citep{}, the naked He-star gets closer in separation for easier He-mass transfer, different configurations of WD+He-star were studied and found XX amount lead to SN Ia themselves, also lots evolved to WD+WD and found XX amount lead to SN Ia as DD scenario \citep{}. When including the WD+He-star configuration to the DD scenario in this one particular advanced simulation, found to make up 2/3 of observed SNe Ia rate \citep{}.

The WD and He-star ``intermediate'' channel also neatly explains the historical delay-time-distribution (DTD) issues stemming from a singular SD or singular DD prescription. Delay time is defined as the time interval from star formation to the thermonuclear runaway explosion (thus a distribution for a population). DTDs predicted by theoretical works not including the WD and He-star channel have large deficits associated with the early (e.g. $\lesssim$ 1 Gyr) and old (e.g. $\gtrsim$ 8 Gyr) epochs of delay time \citep{}. Upon including the WD and He-star pathway, simulations show the DTDs of SNe Ia match better with observations, even more so at the old and early epochs \citep{}.

**Explain the WD+He-star scenario leading to SN Ia as an example, and explain why the helium mass being accreted is more efficient for SN Ia.

**Kinematics of this separate He-star kicked population versus the H-star population. Why distinctly different? Observations support this? (not really) \citet{Tauris2015, Yisikandeer2016} Possible reasons for discrepancy? What would we be looking for, then??

**Unfortunately, simulations also suggest the SN Ia ejecta effects on the ejected companion He-star would also make it difficult to detect large visual differences at late-time observations (as DRs). Examples of accreted ejecta material amounts here with how it would effect observations over short/long time scales.

%Paragraph(s) saying that the SD scenario, in any channel associated with it, implies the companion survives the explosion of the primary - how is it supported by observations or theory? References?

%Effects we should see: examples from simulations (similar to last 3 paragraphs of DD scenario)

%So what do the simulation differences all tell us about what we should expect to see abundances-wise? 

%Kinematics-wise? Detail the differences between composition(DENSITY) of the companion and how that will effect observations (higher density leading to lower separation distance thus faster orbital velocity for same momentum/original star mass). The He-star companions are likely the ones fast enough to catch with large surveys as anomalies, pointed observations only for the slower ones ejected as red giants or main sequence stars.

\subsubsection{Sub-luminous SNe Ia remnants}

A peculiar sub-class of SNe Ia likely produced via the SD scenario have recently been presented in the literature, characterised (among other things) by fainter light curves, lower SN expansion velocities, and lower ejecta mass when compared to Branch-normal Ia events \citep{}. The lower energetics and lower mass ejecta associated with these events, dubbed SNe Iax, are thought to be explained by the partial or full deflagration of a primary WD in the SD scenario (depending on the energy release, \cite{}). This ``failed detonation'' (FD) scenario implies a partial deflagration can leave the primary WD intact and the conditions after the deflagration do not lead to a subsequent detonation (for energies e.g. < ). See \citet{} and \citet{} for discussion on avoiding the transition to detonation. At sufficient enough energies (e.g. > ), the FD scenario implies a full deflagration will propagrate through the entire primary WD and unbind it completely.

What nucleosynthesis is associated with partial/full deflagrations in this scenario? How will that effect the primary? Companion? What might we expect to see here

What kinematics are associated with partial/full deflagrations in this scenario? How might it affect the primary? Companion? What might we expect to see here

Examples in the literature of DRs from this scenario?

\subsection{Observable donor remnant population}



% new ^^^
